First Order Stochastic Optimization with Oblivious Noise

We initiate the study of stochastic optimization with oblivious noise, broadly generalizing the standard heavy-tailed noise setup. In our setting, in addition to random observation noise, the stochastic gradient may be subject to independent oblivious noise, which may not have bounded moments and is not necessarily centered. Specifically, we assume access to a noisy oracle for the stochastic gradient of $f$ at $x$, which returns a vector $\nabla f(\gamma, x) + \xi$, where $\gamma$ is the bounded variance observation noise and $\xi$ is the oblivious noise that is independent of $\gamma$ and $x$. The only assumption we make on the oblivious noise $\xi$ is that $\mathbf{Pr}[\xi = 0] \ge \alpha$ for some $\alpha \in (0, 1)$. In this setting, it is not information-theoretically possible to recover a single solution close to the target when the fraction of inliers $\alpha$ is less than $1/2$. Our main result is an efficient list-decodable learner that recovers a small list of candidates, at least one of which is close to the true solution. On the other hand, if $\alpha = 1-\epsilon$, where $0< \epsilon < 1/2$ is sufficiently small constant, the algorithm recovers a single solution. Along the way, we develop a rejection-sampling-based algorithm to perform noisy location estimation, which may be of independent interest.

==> intro.tex <==
% !TeX root = neurips_2020.tex
\section{Introduction}

A major challenge in modern machine learning systems is to perform inference in the presence of outliers. 
Such problems appear in various contexts, such as analysis of real datasets with natural outliers, 
e.g., in biology~\cite{RP-Gen02, Pas-MG10, Li-Science08}, 
or neural network training,
where heavy-tailed behavior arises from stochastic gradient descent 
when the batch size is small and when the step size is 
large~\cite{hodgkinson2021multiplicative, gurbuzbalaban2021heavy}.
% Specific to noisy gradients
In particular, when optimizing various neural networks, 
there exists strong empirical evidence 
indicating that gradient noise frequently displays heavy-tailed behavior, 
often showing characteristics of unbounded variance. 
This phenomenon has been observed for
fully connected and convolutional neural networks~\cite{simsekli2019tail, gurbuzbalaban2021fractional} 
as well as attention models~\cite{zhang2020adaptive}. 
Hence, it is imperative to develop robust optimization methods for machine learning in terms of both performance and security.

% SETTING; PRIOR WORK WITHOUT OUR NOISE
In this paper, we study robust first-order stochastic optimization 
under heavy-tailed noise, which may not have any bounded moments.
Specifically, 
given access to a noisy gradient oracle for $f(x)$ (which we describe later),
the goal is to find a \textit{stationary point} of the objective function $f : \R^d \rightarrow \R$, 
$f(x) := \E_\gamma [f(\gamma, x)]$, 
where $\gamma$ is drawn with respect to an arbitrary distribution on $\R^d$. 

Previous work on $p$-heavy-tailed noise often considers the case where one has access to 
$\nabla f(\gamma, x)$ such that 
$\E_\gamma [\nabla f(\gamma, x)] = \nabla f(x)$ and 
$\E_\gamma[\norm{\nabla f(\gamma, x)-\nabla f(x)}^p] \leq \sigma^p$
for $p = 2$ \cite{nazin2019algorithms, gorbunov2020stochastic}, 
and recently for $p \in (1, 2]$~\cite{cutkosky2021high, sadiev2023high}.
In contrast, \cite{DiakonikolasKKLSS2018sever} investigates a more challenging noise model 
in which a small proportion of the sampled functions $f(\gamma, x)$ 
are arbitrary adversarial outliers. 
In their scenario, they have full access to the specific 
functions being sampled and can eventually eliminate all but the least harmful 
outlier functions. 
Their algorithm employs robust mean estimation techniques to 
estimate the gradient and filter out the outlier functions.
Note that their adversarial noise model requires that at least half of the samples are inliers. 
% while they also have access to the
% specific functions being sampled, and hence can eventually 
% remove all the outlier functions. 

This work aims to relax the distributional assumption of heavy-tailed noise 
such that the fraction of outliers can approach one, and do not have any bounded moment constraints
while keeping optimization still computationally tractable.
Thus, we ask the following natural question:
\begin{center}
{\em 
% Are there realistic noise models for first-order optimization in which\\
% efficient learning is possible without strong distributional assumptions?
What is the weakest noise model for optimization in which
efficient learning is possible,\\
while allowing for strong corruption of almost all samples?
}
\end{center}
% \snote{Something like: What is the weakest noise model, 
% allowing for $> 1/2$ fraction of the samples being arbitrarily corrupted
% where efficient learning is possible?}
% \jnote{maybe, but i wouldn't put 1/2 in this question. 'arbitrarily' is a vague word too.}
% \snote{How about: What is the weakest noise model, 
% allowing for almost all the samples being corrupted
% where efficient learning is possible?}

% OUR PROBLEM
In turn, we move beyond prior heavy-tailed noise models with bounded moments 
and define a new noise model for first-order optimization, 
inspired by the oblivious noise model studied in the context of regression~\cite{BhatiaJK15, d2020regress}.
We consider the setting in which the gradient oracle returns
noisy gradients whose mean may not be $\nabla f(x)$, and in fact, may not even exist. 
The only condition on our additive noise distribution of $\xi$ is that with probability at least $\alpha$,
oblivious noise takes the value zero. Without this, the optimization problem would become intractable.
Notably, oblivious noise can capture any tail behavior that arises from independent $p$-heavy-tailed noise.

We now formally define the oblivious noise oracle below.


\begin{definition}[Oblivious Noise Oracle]
\label{def:oblivious_noise_oracle}
We say that an oracle $\cO_{\alpha, \sigma, f}(x)$ is an oblivious-noise oracle,
if, when queried on $x$, the oracle returns $\nabla f(\gamma, x) + \xi$ 
where $\gamma$ is drawn from some arbitrary distribution $Q$ and $\xi$ is drawn from $D_\xi$ independent of $x$ and $\gamma$, satisfying  $\Pr_{\xi \sim D_\xi}[\xi = 0] \geq \alpha$. The distribution $Q$ satisfies $\E_{\gamma \sim Q}[\nabla f(\gamma, x)] = \nabla f(x)$ 
and $\E_{\gamma \sim Q}[\norm{\nabla f(\gamma, x) - \nabla f(x)}^2] \leq \sigma^2$.
% \new{while $\xi$ (independent of $\gamma$ and $x$) satisfies} .
\end{definition} 

% DO EVERYTHING FOR STATIONARITY -- SEVER

% EXPLAINING OBLIVIOUS NOISE -- SEVER

% This is in line with other work which as studied this noise model in the 
% context of mean-estimation \cite{}, linear regression \cite{} and so on.

Unfortunately, providing an approximate stationary point 
$\widehat x$ such that $\|\nabla f(\widehat x)\| \le \eps$,  
for some small $\eps > 0$, is information-theoretically impossible when $\alpha \le 1/2$. 
To see this, consider the case where $\Pr_\gamma [\gamma = 0] = 1$
and the function $f(0, x) = x^2$. 
If $\xi$ follows a uniform distribution over the set $\{-2, 0, 2\}$,
when we query the oracle for a gradient at $x$, we will observe a uniform distribution
over $\{2x-2, 2x, 2x+2\}$.
This scenario cannot be distinguished from a similar situation where the objective is to minimize 
$f(0, x) = (x-1)^2$, and $\xi$ follows a uniform distribution over $\{0, 2, 4\}$.

To address this challenge, we allow our algorithm to work in the \textit{list-decodable} setting, implying that it may return 
a small list of candidate solutions
such that one of its elements $\widehat x$ satisfies $\|\nabla f(\widehat x)\| \le \eps$.
We now define our main problem of interest.

\begin{definition}[List-Decodable Stochastic Optimization]\label{def:GNM_prob}
The problem of
% $(\eta, \alpha, \sigma, f)$-
List-Decodable Stochastic Optimization with oblivious noise is defined as follows:
For an $f$ that is $L$-smooth and has a global minimum, given access to $\cO_{\alpha, \sigma, f}(\cdot)$ as defined in \Cref{def:oblivious_noise_oracle}, 
the goal is to output a list $\cL$ of size $s$ 
such that $\min_{\widehat x \in \cL} \norm{ \nabla f(\widehat x) } \leq \eps$. 
\end{definition}

\subsection{Our Contributions}

As our main result, we demonstrate the equivalence between 
list-decodable stochastic optimization with oblivious noise
and list-decodable mean estimation (LDME), which we define below.

\begin{definition}[List-Decodable Mean Estimation]\label{def:LDME_alg}
Algorithm $\cA$ is an $(\alpha, \beta, s)$-LDME
algorithm for $\cD$ (a set of candidate inlier distributions) 
if with probability $1-\delta_{\cA}$,  
it returns a list $\cL$ of size $s$ 
such that 
$\min_{\hat \mu \in \cL} \norm{\hat \mu - \E_{x \sim D}[x]} \leq \beta$ for $D \in \cD$
when given $m_\cA$ samples $\{z_i + \xi_i \}_{i=1}^{m_\cA}$
for $z_i \sim D$ and $\xi_i \sim D_\xi$ where $\Pr_{\xi \sim D_\xi}[\xi = 0] \geq \alpha$.
If $1-\alpha$ is a sufficiently small constant less than $1/2$, then $s = 1$. 
% \jnote{last line slightly modified.}
\end{definition}

We define $\cD_\sigma$ to be the following set of distributions 
over $\R^d$: $\cD_\sigma := \{ D \mid \E_{D}[\norm{x - \E_D[x]}^2] \leq \sigma^2\}$.
We also use $\tilde O(\cdot)$ to hide all log factors in $d, 1/\alpha, 1/\eta, 1/\delta$, where
$\delta$ denotes the failure probability and $\eta$ is a multiplicative parameter we use in our algorithm.

Our first theorem shows that if there exists 
an efficient algorithm for the problem 
of list-decodable mean estimation
and an inexact learner (an optimization method using inexact gradients), 
there is an efficient algorithm for list-decodable stochastic optimization. 

\begin{theorem}[List-Decodable Stochastic Optimization $\rightarrow$ List-Decodable Mean Estimation]
\label{thm:LDSO_reduce_to_LDME_informal}
Suppose that for any $f$ having a global minimum and being $L$-smooth, the algorithm $\cA_G$,
given access to $g_x$ satisfying $\norm{g_x - \nabla f(x)} \leq O(\eta \sigma)$,
recovers $\hat x$ satisfying $\norm{\nabla f(\hat{x}) } \leq O(\eta \sigma)+\eps$ in time $T_G$.
% \jnote{Since we "suppose" this here, maybe we don't need to mention the global minimum / black-box optimization assumptions. SK: I think we might not mathematically need this, but we should be a little bit more explicit.}
Let $\cA_{ME}$ be an $(\alpha, O(\eta \sigma), s)$-LDME algorithm 
for $\cD_\sigma$.
% and $\cA_G$  be an $(\beta',\eps)$-inexact-learner for  $\beta' = \beta + O(\eta \sigma)$.
Then, there exists an algorithm (\Cref{alg:main_algo}) which uses $\cA_{ME}$ and $\cA_G$,
makes \new{ $m = m_{\cA_{ME}} + \tilde O(T_G \cdot (O(1)/\alpha)^{2/\eta}/\eta^5)$ }
queries to $\cO_{\alpha, \sigma, f}$, 
\new {runs in time $T_G\cdot\poly(d, 1/\eta, (O(1)/\alpha)^{1/\eta}, \log(1/\delta \eta \alpha))$, }
and returns a list $\cL$ of $s$ candidates  satisfying
$\min_{x \in \cL} \norm{ \nabla f(x)} \leq O(\eta \sigma) + \eps$
with probability $1-\delta_{\cA_{ME}}$.
% \jnote{the $\epsilon$ is weird here. also $\beta$'s role is unclear in the final guarantee.}
% \snote{the learner is a beta + whatever, eps learner.. what would you rather have? 
% we could remove beta entirely from the statement perhaps.}
\end{theorem}

To achieve this reduction, we develop an algorithm capable of determining 
the translation between two instances of a distribution by utilizing samples 
that are subject to additive noise. 
It is important to note that the additive noise can differ for each set of samples. 
As far as we know, this is the first guarantee of its kind for estimating the location of a distribution, 
considering the presence of noise, sample access, and the absence of density information.

% To perform this reduction, we rely on an algorithm that is able to 
% identify the translation between two copies of a distribution 
% give access to additively noisy samples of these distributions,
% where the additive noise might be different for each of the sample sets. 
% To this best of our knowledge, this is the first such guarantee for noisy finite-sample
% location estimation only given sample-access and without access to the density of the distribution.

\begin{theorem}[Noisy Location Estimation]\label{thm:loc-est_informal}
Let $\eta \in (0, 1)$ and let $D_\xi, D_z, D_{z'}$ be distributions such that 
$\Pr_{\xi \sim D_\xi}[\xi = 0] \geq \alpha$ and 
$D_z, D_{z'}$ are possibly distinct mean zero distributions with variance bounded by $\sigma^2$.
Then there is an algorithm (\Cref{alg:loc_algo}) which, 
for unknown $t \in \R^d$,
takes $m = \tilde O((1/\eta^5)(O(1)/\alpha)^{2/\eta})$
% \jnote{Why geq?}
% (1/\eta^3 \alpha^4) \log(1/\eta \alpha \delta)$
samples $\{\xi_i + z_i + t\}_{i=1}^m$ and $\{\tilde \xi_i + z'_i\}_{i=1}^m$, where $\xi_i$ and $\tilde \xi_i$ are drawn independently from $D_\xi$ and $z_i$ and $z'_i$ are drawn from $D_z$ and $D_{z'}$ respectively,
runs in time $\poly(d, 1/\eta, (O(1)/\alpha)^{1/\eta}, \log(1/\delta \eta \alpha))$, 
and with probability $1-\delta$ recovers $t'$ such that $|t-t'| \le O(\eta \sigma)$.    
\end{theorem}

The fact that there exist algorithms for list-decodable mean estimation with the inliers coming from $\cD_\sigma$ allows us to get concrete results for list-decodable stochastic optimization. 

Conversely, we show that if we have an algorithm for 
list-decodable stochastic optimization, then we also get an algorithm
for list-decodable mean-estimation. 
This in turn implies, via \Cref{fact:list_decoding_D_sigma}, 
that an exponential dependence on $1/\eta$ is necessary in the list-size
if we want to estimate the correct gradient
up to an error of $O(\eta \sigma)$ when the inliers are drawn from some distribution in $\cD_\sigma$. 

\begin{theorem}[List-Decodable Mean Estimation $\rightarrow$ List-Decodable Stochastic Optimization]
\label{thm:LDME_reduce_to_LDSO_informal}
Assume there is an algorithm for 
List-Decodable Stochastic Optimization with oblivious noise
that runs in time $T$ and makes $m$ queries to $\cO_{\alpha, \sigma, f}$,
and returns a list $\cL$ of size $s$ containing $\wh x$ satisfying $\norm{  f(\wh x) } \leq \eps$.
Then, there is an $(\alpha, \eps, s)$-LDME
algorithm for $\cD$
that runs in time $T$, queries $m$ samples, and returns a list of size $s$.
\end{theorem}

If $\alpha = 1-\eps$, where $0< \eps< 1/2$ is at most a sufficiently small
constant, the above theorems hold for the same problems, but with the constraint
that the list is singleton. 

\input{NeurIPS/prior_work}

\subsection{Technical Overview}

For ease of exposition, we will make the simplifying assumption that the observation noise is bounded between $[-\sigma, \sigma]$.
Let $y$ and $y'$ be two distinct mean-zero noise distributions, both bounded within the range $[-\sigma, \sigma]$.
Define $\xi$ to be the oblivious noise drawn from $D_\xi$, 
satisfying $\Pr[\xi = 0] \geq \alpha$.
Assume we have access to the distributions (i.e., we have infinite samples).

\paragraph{Stochastic Optimization reduces to Mean Estimation.}
In \Cref{thm:LDSO_reduce_to_LDME_informal}, we show how we
can leverage a list-decodable mean estimator to address the challenge 
of list-decodable stochastic optimization with oblivious noise (see \Cref{alg:main_algo}). 
The key idea is to recognize that we can a generate list of gradient estimates, and update this list such that 
one of the elements always closely approximates the true gradient in $\ell_2$ norm at the desired point. 

The algorithmic idea is as follows:
First, run a list-decodable mean estimation algorithm on the noisy gradients at $x_0=0$ 
to retrieve a list $\cL$ consisting of $s$ potential gradient candidates. 
This set of candidates contains at least one element which closely approximates $\nabla f(0)$.
    
One natural approach at this stage would be to perform a gradient descent step for each of the $s$ gradients, 
and run the list-decodable mean estimation algorithm again
to explore all potential paths that arise from these gradients. 
However, this naive approach would accumulate an exponentially large number of candidate solutions. 
We use a location-estimation algorithm to tackle this issue. 

We can express $f(\gamma, x)$ as $f(x) + e(\gamma, x)$ where $\E_\gamma[e(\gamma, x)] = 0$
and $\E_\gamma [\norm{e(\gamma, x)}^2 ] < \sigma^2$. 
When we query $\cO_{\alpha, \sigma, f}(\cdot)$ at $x$, 
we obtain samples of the form $\nabla f(x) + \xi + \nabla e(\gamma, x)$,
i.e., samples from a translated copy of the oblivious noise distribution convolved with 
the distribution of $\nabla e(\gamma, x)$. We treat the distribution of $\nabla e(\gamma, x)$ as observation noise.
The translation between the distributions of our queries to $\cO_{\alpha, \sigma, f}(\cdot)$ at $x$ and $0$ correspond to $\nabla f(x) - \nabla f(0)$. 
To update the gradient, it is sufficient to recover this translation accurately. 
By doing so, we can adjust $\cL$ by translating each element while maintaining the accuracy of the estimate.
% that maintains the accuracy of the gradient  the correct gradient at the initial point $0$ remains the correct gradient at the current point $x$.
% \snote{changed para, more readable?}

Finally, we run a first-order learner for stochastic optimization using these gradient estimates. 
We select and explore $s$ distinct paths, with each path corresponding to an element of $\cL$ obtained earlier. 
Since one of the paths always has approximately correct gradients, this path will converge to a stationary point 
in the time that it takes for the first-order learner to converge.

% We now discuss how to perform location estimation.

\paragraph{Noisy Location Estimation in 1-D.} 
The objective of noisy location estimation is to retrieve the translation 
between two instances of a distribution by utilizing samples that are subject to additive
mean-zero and bounded-variance noise. 

In \Cref{lem:1d-loc-est}, we establish that if \Cref{alg:loc_algo1d} 
is provided with a parameter $\eta \in (0, 1)$ and samples from the distributions of
$\xi + y$ and $\tilde \xi + y' + t$, 
it can recover the value of $t$ within an error of $O(\eta \sigma)$. 
Here $\xi$ and $\tilde \xi$ are independent draws from the same distribution.

Observe that in the absence of additive noise $y$ and $y'$, 
$t$ can be estimated exactly by simply taking the median of a sufficiently large number of pairwise differences 
between independent samples from $\xi$ and $\tilde \xi + t$. 
This is because the distribution of $\tilde \xi - \xi$ 
% where both $\xi$ and $\tilde \xi$ follow the same oblivious noise distribution, 
is symmetric at zero and $\Pr[\tilde \xi - \xi=0] = \alpha^2$.
However, with unknown $y$ and $y'$, this estimator is no longer consistent
since the median of zero-mean and $\sigma$-variance random variables can be
as large as $O(\sigma)$ in magnitude.
In fact, \Cref{claim:rough_estimate} demonstrates that for the setting we consider
the median of $\xi + y$ can as far as $O(\sigma/\sqrt{\alpha})$ far from the mean of $\xi$. 
However, it does recover a rough estimate $t'_r$ such that $|t-t'_r| \le O(\sigma/\sqrt{\alpha})$.

Consequently, our approach starts by using $t'_r$ as the estimate for $t$, 
and then iteratively improving the estimate by mitigating the heavy-tail influence of $\xi$. 
Note that if $\xi$ did not have heavy tails, then we could try to directly compute $t = \E[\xi + y' + t] - \E[\xi + y]$.
Unfortunately, due to $\xi$'s completely unconstrained tail, $\xi$ may not even possess a well-defined mean.
% if we were able to compute the expectations of the distributions, 
% then $\E[\xi + y + t] - \E[\xi + y']= t$
% since the means of $y$ and $y'$ are both $0$.
% However, the distribution of $\xi$ may not possess a well-defined mean, 
% and even if it did, 
% it might require a very large sample size to achieve convergence or concentration.
Nonetheless, if we are able to condition $\xi$ to a bounded interval, 
we can essentially perform the same calculation described above. 
% the independence of $y, y'$ and $\xi$ allows us to perform the same calculation.
In what follows, we describe one step of an iterative process to improve our estimate of $t$. 

\paragraph{Rejection Sampling.}
Suppose we have an initial rough estimate of $t$, given by $t'_r$ such that $|t'_r - t| < A\sigma$. 
We can then re-center the distributions to get $\xi + z$ and $\xi + z'$, 
where $z$ and $z'$ have means of magnitude at most $A\sigma$, and have variance that is $O(\sigma)$. 
\Cref{claim:fine_estimate} then shows that we can refine our estimate of $t$.
It does so by identifying an interval $ I = [-k\sigma,k\sigma]$ around $0$ such that the addition of either $z$ or $z'$ to $\xi$ 
does not significantly alter the distribution's mass within or outside of $I$. 
We show that since $z, z'$, and $\xi$ are independent, 
the $I$ that we choose satisfies 
% that the difference between the conditional expectations 
$\E[\xi + z' \mid \xi + z' \in I]-\E[\xi + z \mid \xi + z \in I]=\E[\xi + z' \mid \xi \in I] - \E[\xi + z \mid \xi \in I] \pm \eta A = \E[z'] - \E[z] \pm \eta A$ for some $\eta < 1$.

To see that such an interval $I$ exists, we will show that for some $i$, there are
pairs of intervals $ (A\sigma i, (i+1)A\sigma]$ and $ [-(i+1)A\sigma , -iA\sigma )$ which 
contain a negligible mass with respect to $\xi$. 
Since $z$ and $z'$ can move mass by at most $(A+1)\sigma$ with high probability, 
it is sufficient to condition on the interval around $0$ which is contained in this pair of intervals.
Since we do not have access to $\xi$, 
we instead search for pairs of intervals of length $O(A\sigma)$ which have negligible mass 
with respect to both $\xi + z$ and $\xi + z'$, which suffices. 

To do this, we will demonstrate an upper bound $\tP(i)$ on the mass crossing the $i^{th}$ pair of intervals described above. This will satisfy $\sum_i \tP(i) = C'$ for some constant $C'$. 
% denot$:= 
% \Pr[\xi+z \in \sigma (i-4 \cdot 12, i+4\cdot 12] \cup \sigma [\new{-i}-4 \cdot 12, -i+4\cdot 12)] + 
% \Pr[\xi+z' \in \sigma (i-4\cdot 12, i+4\cdot 12] \cup \sigma [\new{-i}-4\cdot 12, -i+4\cdot 12)]$ be an upper bound on the mass described above. 
% and each interval of size $\sigma$ is overcounted at most a constant number of times.

To show that this implies there is an interval of negligible mass, 
we aim to demonstrate the existence of a $k \in \mathbb N$ such that $k \tP(k) \leq \eta$. 
We will do this through a contradiction. 
Suppose this is not the case for all $i \in [0, k]$, then $\sum_{i=0}^k \tP(i) \geq \eta \sum_{i=0}^k (1/i)$. 
If $k \geq \exp(10 C'/\eta)$, we arrive at a contradiction because 
the right-hand side is at least $\eta \sum_{i=0}^{k} (1/i) \geq \eta \log(\exp(10 C/\eta)) > 10C'$, 
while the left-hand side is bounded above by $C$. 

\Cref{claim:tildeP} demonstrates, via a more involved and finer analysis, 
that for the bounded-variance setting where intervals very far away can contribute to mass crossing $A\sigma i$,
there exists an $k$ such that  $k \tP(k) \leq \eta \Pr[\abs{\xi} < A \sigma k]$, 
and that taking the conditional mean restricted to the interval $[-kA\sigma, kA\sigma]$ allows us to improve our estimate of $t$. 
Here $\tP(k)$ denotes an upper bound on the total probability mass that crosses intervals described above. 

% \new{In the example above, our noise is bounded by $\sigma$ in magnitude, and so $z$ and $z'$ cannot distort the median more than $O(\sigma)$. 
% However, in general, they might distort the median by up to $O(\sigma/\sqrt{\alpha})$. What is described above will amount to a single step that makes progress, but needs to be repeated $\log(1/\alpha)$ times to converge. }

\paragraph{Extension to Higher Dimensions.}
In order to extend the algorithm to higher dimensions, 
we apply the one-dimensional algorithm coordinate-wise, but in a randomly chosen coordinate-basis. 
% However, a challenge arises from the fact that the algorithm requires a good estimate of 
% the standard deviation for each coordinate, which is not known in advance.
\Cref{lem:loc_est} uses the fact that representing the distributions in a randomly
rotated basis ensures that, with high probability, the inlier distribution
will project down to each coordinate with a variance of $O(\sigma\sqrt{\log(d)}/\sqrt{d})$
to extend \Cref{lem:1d-loc-est} to higher dimensions. 

\paragraph{Mean Estimation reduces to Stochastic Optimization.}
In \Cref{thm:LDME_reduce_to_LDSO_informal} we show that the problem of list-decodable mean 
estimation can be solved by using list-decodable stochastic optimization 
for the oblivious noise setting.
This establishes the opposite direction of the reduction 
to show the equivalence of list-decodable mean estimation
and list-decodable stochastic optimization.

The reduction uses samples from the list-decodable mean estimation problem 
to simulate responses from the oblivious oracle to queries at $x$.
Let the mean of the inlier distribution be $\mu$. 
If the first-order stochastic learner queries $x$, 
we return $x + s$ where $s$ is a sample drawn from the list-decodable mean-estimation problem. 
These correspond to possible responses to the queries when $f(x) = (1/2) \norm{x + \mu}^2$, where $\mu$ is the true mean. The first-order stochastic learner learns a $\wh \mu$ from a list $\cL$ such that $\norm{\nabla f(\wh \mu)} = \norm{\wh \mu + \mu} \le \eps$; then the final guarantee of the list-decodable mean estimator follows by returning $-\cL$ which contains $-\wh \mu$.

==> old.tex <==
Rejection sampling kinda thing for location estimation. 

\begin{proof}
Note that if we could take expectations of the distributions, then $\E[\xi + y + x] - \E[\xi + y'] = x$, and we would be done. 
However $Q$ might not even have a mean, and even if it did, might require far too many samples to concentrate.
To address this, we will perform rejection sampling such that the resulting distribution
has sub-exponential tails, and hence concentrates, and the difference remains approximately unaffected.

The idea is simple, we first identify roughly the same relative position in both distributions,
then we multiply the pdf of the distribution with $\exp(-\eps |t-c|)$ where $c$ is the position,
and then normalize. This will result in sub-exponential tails for the distribution after rejection sampling.

To roughly identify the same relative position in both distributions, do the following: 
For the distributions $\xi + y$ and $\xi + y'$, 
consider the leftmost interval of length $20 \sigma$ containing a mass of $\alpha$.
Let these be $I$ and $I'$. 
In both cases, we know that at least one such interval exists, since $\xi + y'$ 
places a mass of $\alpha$ in $[-10\sigma, 10\sigma]$ and the same holds for 
$\xi + y + x$ for the interval $x + [-10\sigma, 10\sigma]$.
Let $c, c'$ be the centers of $I$ and $I'$. 
Since the quantiles at which $I$ and $I'$ occur are the same, upto an error of $O(\sigma)$ \snote{check}, 
we see that $\abs{c - x} < O(\sigma)$ and $\abs{c' - 0} < O(\sigma)$.

We now compute the difference of the centered new distributions.
To this end, we need the following lemmas

\begin{lemma}
\label{lem:reject_samp}
Let $z \sim D$ be a random variable with mean $0$ and variance $\sigma'^2$. 
Suppose $\sigma' \sqrt{\eps} < 1$ and let $\pE$ denote the distribution after rejection sampling by reducing the mass of $z$ at $x$ by $\exp(-\eps |x|)$. 
Then $\pE[z] = O(\sqrt{\eps} \sigma')$.
\end{lemma}
\begin{proof}
The proof follows from the following facts and the law of total probability.
\begin{enumerate}
    \item $\pE[z \mid \abs{z} < \sigma'/\sqrt{\eps}] = O(\sigma' \sqrt{\eps})$.\label{item:E_bound_in}
    \item If $t > 0$ then $\widetilde \Pr[\abs{z} >t] < O(\sigma'^2/t^2)$.\label{item:P_bound}
    \item $\pE[z \mid \abs{z} > \sigma'/\sqrt{\eps}] = O(\sigma'/\sqrt{\eps})$.\label{item:E_bound_out}
\end{enumerate}
Putting these three together, we get 
\begin{align*}
\pE[z] &= (1-\widetilde \Pr[\abs{z} > \sigma'/\sqrt{\eps}]) ~\pE[z \mid \abs{z} < \sigma'/\sqrt{\eps}] 
+ \widetilde \Pr[\abs{z} > \sigma'/\sqrt{\eps}] ~\pE[z \mid \abs{z} > \sigma'/\sqrt{\eps}]\\
&\leq (1-\eps) O(\sigma' \sqrt{\eps}) + O(\eps \sigma'/\sqrt{\eps}) = O(\sigma' \sqrt{\eps}). 
\end{align*}


Proof of \Cref{item:E_bound_in}:
\begin{align*}
\pE[z \mid \abs{z} < \sigma'/\sqrt{\eps}] 
&= \frac{\int_{ \abs{z} < \sigma'/\sqrt{\eps}} z \exp(-\eps |z|) \mu_D(x)}{ \int_{ \abs{z} < \sigma'/\sqrt{\eps}} \exp(-\eps |z|) \mu_D(x)}\\
&< \exp(\sqrt{\eps} \sigma') \frac{\int_{ \abs{z} < \sigma'/\sqrt{\eps}} z ~\mu_D(x)}{ \int_{ \abs{z} < \sigma'/\sqrt{\eps}} ~\mu_D(x)} \\
&= \exp(\sqrt{\eps} \sigma') \E[z \mid \abs{z} < \sigma'/\sqrt{\eps}]\\
&<  O(\sigma' \sqrt{\eps})
\end{align*}
Where the final inequality follows from the fact that the mean 
of a bounded variance random variable can change by at most $\sigma' \sqrt{\eps}$ 
if it is missing an $\eps$ fraction of the mass, and the fact that $\sqrt{\eps} \sigma' < 1$. 

Proof of \Cref{item:P_bound}:
\begin{align*}
\widetilde \Pr[\abs{z} > t] 
&=\frac{\int_{ \abs{z} >t} \exp(-\eps |z|) ~d\mu_D(x)}{ \int \exp(-\eps |z|) ~d\mu_D(x)}\\
&< \frac{\int_{ \abs{z} > t} ~d\mu_D(x)}{ \int \exp(-\eps |z|) ~d\mu_D(x)}\\
&< O(\sigma'^2/t^2)
\end{align*}
Where the final inequality follows by Chebyshev on the numerator, 
and the fact that the denominator is lower bounded by a constant. \snote{check}

Proof of \Cref{item:E_bound_out}:
\begin{align*}
\pE[\abs{z} \mathbf{1}( \abs{z} > \sigma'/\sqrt{\eps})] 
&= \int_{ t} \widetilde \Pr[\abs{z} \mathbf{1}( \abs{z} > \sigma'/\sqrt{\eps}) > t]~dt\\
&= \int_{ t} \widetilde \Pr[\abs{z} \mathbf{1}( \abs{z} > \sigma'/\sqrt{\eps}) > \max(t, \sigma'/\sqrt{\eps})]~dt\\
&= O(\sigma' \sqrt{\eps}) + \int_{t >  \sigma'/\sqrt{\eps}} \widetilde \Pr[\abs{z} > t]~dt\\
&< O(\sigma' \sqrt{\eps})
\end{align*}
Where the final few inequalities are a consequence \Cref{item:P_bound}. 
\end{proof}
\end{proof}

\begin{lemma}\label{lem:shifted_reject_samp}
Let $z \sim D$ be a random variable with mean $0$ and variance $\sigma'^2$. 
Suppose $\sigma' \sqrt{\eps} < 1$ and let $\pE$ denote the distribution after rejection sampling by reducing the mass of $z$ at $x$ by $\exp(-\eps |x + \xi|)$. 
Then $\pE[z + \xi] = $.
\end{lemma}
\begin{proof}
    Let $Z = \int \exp(-\eps |x + \xi|)  ~d\mu_D(z)$ be the normalizing constant.
    Note that $Z >  \exp(\eps |\xi|)\int \exp(-\eps |x|)  ~d\mu_D(z)$ and 
    $Z >  \exp(-\eps |\xi|) \int \exp(\eps |z|) ~d\mu_D(z)$
    We first show the upper bound.
    \begin{align*}
        \pE[z + \xi] &= (1/Z)~\int (z + \xi) \exp(-\eps |z + \xi|) ~d\mu_D(z)\\
        &= (1/Z)~\int \xi\exp(-\eps |z + \xi|) ~d\mu_D(z)
        + (1/Z)~\int z\exp(-\eps |z + \xi|) ~d\mu_D(z)\\
         % &= (1/Z)~\int \xi\exp(-\eps |z + \xi|) ~d\mu_D(z)
        % + (1/Z)~\int z\exp(-\eps |z + \xi|) ~d\mu_D(z)\\
        &< (1/Z)~\xi\exp(-\eps |\xi|)\int\exp(\eps |z|)~d\mu_D(z)
        + (1/Z)~\exp(\eps |\xi|) \int z\exp(-\eps |z|) ~d\mu_D(z)
    \end{align*}
\end{proof}

\begin{lemma}[Finding Common Representative Quantile]\label{lem:rep_quantile_varying_D}
Let $D_1, D_2$ be two distributions with mean $0$ and variance bounded by $\sigma^2$.
Let $\cD_i := \alpha D_i + (1-\alpha) Q$.
Then in $m = O(\log(1/\alpha \delta)/\alpha^2)$ samples and time $O(m/\alpha)$
we can identify an interval $I'$ of length $200 \sigma$ 
containing mass at least $0.96 \alpha$ with respect to $\cD_1$ and $\cD_2$.
Also, if $p$ is the left-most point of the interval $I'$, then 
$\abs{\Pr_{z \sim \cD_1}[z < p] - \Pr_{z \sim \cD_2}[z < p]} < 0.04\alpha$. 
\end{lemma}
\begin{proof}
Since $\E_{D_j}[x^2] \leq \sigma^2$ for $j \in \{1, 2\}$,
we know that $\Pr_{x \sim D_j}[\abs{x} > 100 \sigma] < 10^{-4}$ for any such distribution. 
This implies that the mixture $\cD_j$ places a mass of $(1-10^{-4})\alpha$
on the interval $I = [-100 \sigma, 100 \sigma]$. 

Consider $P = \{ 10^{-6}\alpha, 2 ~10^{-6}\alpha, 3 ~10^{-6}\alpha \dots, 1 \}$. 
By Hoeffding's inequality \Cref{lem:hoeffding} and a union bound, 
we know that in $m = O(\log(1/\alpha \delta)/\alpha^2)$ samples from $\cD_1$ and $\cD_2$, 
we can find $x_1, \dots, x_{10^6/\alpha}$ such that for each $x_i$ 
there is a $\hat p$ satisfying $\Pr_{z \sim \cD_1}[z < x] < \hat p$ such that $\abs{\hat p - (i/10^4) \alpha} \leq \alpha/(2 ~10^4)$.

Consider an interval of length $200 \sigma$ centered at each of these $x_i$. 
If there is an interval which contains mass $> (1-10^{-3}) \alpha$
with respect to $\cD_1$, then choose this interval $I'$. 
With probability $1-\delta$ it will also have mass $> 0.1 \alpha$ with respect to $\cD_2$.

To see the final claim, observe that 
$\Pr_{z \sim \cD_i} [z \in I'] 
= \alpha \Pr_{z \sim D_i}[z \in I'] + (1-\alpha) \Pr_{z \sim Q}[z \in I']$.
This implies, that if $\Pr_{z \sim \cD_1} [z \in I'] > (1-10^{-3}) \alpha$ then either,
$\Pr_{z \sim D_1}[z \in I'] > (1-10^{-2})$ or $\Pr_{z \sim Q}[z \in I'] > (10^{-2} - 10^{-3}) \alpha / (1-\alpha)$. 
If the second is true, the both $\cD_1$ and $\cD_2$ and place a mass of at least 
$(10^{-2} - 10^{-3}) \alpha$ on the interval $I'$.
If $\Pr_{z \sim D_1}[z \in I'] > (1-10^{-2})$ then $\Pr_{z \sim D_2} [z \in I']$
If the first is true, then this means at most $10^{-2}$ mass is left over, 
implying that $I'$ includes $[-5\sigma, 5\sigma]$, since the mass outside this region is $> 0.1$. 
This implies that $\Pr_{z \sim D_2} [z \in I'] > 1-(1/25)$,
implying that $\cD_2$ places a mass of $>0.96 \alpha $ in this region.

Additionally, let $p$ be the leftmost point of $I'$.
Then $\abs{\Pr_{z \sim \cD_1}[z < p] - \Pr_{z \sim \cD_2}[z < p]} < \alpha \abs{\Pr_{z \sim D_1}[z < p] - \Pr_{z \sim D_2}[z < p]} < 0.04 \alpha$, 
implying that the intervals start at the same quantile upto $0.04 \alpha$.
\end{proof}

%INTRO OUR RESULTS
% $\alpha D_x + (1-\alpha) Q$ such that $\E_{z \sim D_x} [z] = \nabla f(x)$ and $Q$ might be arbitrary.
% The idea is to use the robust / list-decodable mean estimation algorithm to either recover a list (possibly of size 1), 
% such that one of the candidates is close to the true mean of $D_x$.
% A natural idea is to start at $0$, and generate a list of points using the gradient update from the inexact learner \snote{correct term?} applied to the list generated by the mean estimation algorithm.
% Since there will always be one good gradient estimate, there will be one sequence of points which will satisfy the guarentees of the learner. 
% Unfortunately, this could potentially lead to exponentially many paths to explore, and the final list size could be very large. 
% \snote{Should we also talk about how there might be some ways using reproducible list-decodable mean estimation algorithms?}

% To circumvent this, we observe that at $x$ we see samples from $\alpha D_x + (1-\alpha) Q$, 
% which can be thought of as $\nabla f(x) + a \xi'_x + (1-a) \xi$ where $\xi'_x$ could depend on $x$,
% but has mean $0$ and $\E[\norm{\xi'_x}^2] < \sigma^2$, $\xi \sim Q$, and $a = 1$ with probability $\alpha$ and $0$ otherwise. 
% This implies that if we query the mixture oracle at $0$ and $x$, we ``essentially'' have 
% two distributions which are shifted by $\nabla f(0) - \nabla f(x)$ with respect to each other. 


% Unfortunately, when we have a list, such that one of the candidates in the list is good




% To design an acceptable oracle for then $(\beta, \eps)$-inexact-learner we need to
% simulate the correct gradient 
% When queried at two points $x$ and $x'$, the oracle $\cO_{\alpha, \sigma, f}^m(\cdot)$


==> prior_work.tex <==
\subsection{Related Work}\label{sec:related_work}

Given the extensive robust optimization and estimation literature, we focus on the most relevant work.

\paragraph{Optimization with Heavy-tailed Noise}
There is a wealth of literature on both the theoretical and empirical
convergence behavior 
of stochastic gradient descent (SGD) for both convex and non-convex problems, 
under various assumptions on the stochastic gradient (see, e.g.,~\cite{hardt2016train, wang2021convergence} and references within).
% \snote{Mention how papers have said noise might be useful in some non-convex settings so that we don't mislead.} 
% \snote{is there a barrier to performing list-decodable learning with a $[1, 2)$ moment bounded?}
However, the noisy gradients have shown to be problematic when training ML models~\cite{shen2019learning, zhang2020adaptive}, hence necessitating robust optimization algorithms.

From a theoretical point of view, several noise models have been proposed to account for inexact gradients. 
A line of work~\cite{d2008smooth, so2013nonasymptotic, devolder2014first, cohen2018acceleration} studies the effects of inexact gradients to optimization methods in terms of error accumulation.
For instance,~\cite{devolder2014first} demonstrates that, given an oracle that outputs an arbitrary perturbation of the true gradient,
the noise can be determined adversarially
to encode non-smooth problems.
Alternatively, many recent works~\cite{lan2012optimal, gorbunov2020stochastic, cutkosky2021high, mai2021stability, sadiev2023high} have studied
$p$-heavy-tailed noise,
an additive stochastic noise to the true gradient
where one has access to 
$\nabla f(\gamma, x)$ such that $\E_\gamma [\nabla f(\gamma, x)] = \nabla f(x)$ and $\E_\gamma[\norm{\nabla f(\gamma, x)-\nabla f(x)}^p] \leq \sigma^p$.
For instance,~\cite{sadiev2023high} propose and analyze a variant of clipped-SGD 
to provide convergence guarantees for when $p\in (1,2]$. However, these noisy oracles, whether deterministic or stochastic, assume bounded norm or moments on the noise, an assumption that is not present in the oblivious noise oracle.

% On the other hand, \citet{CSV17, DiakonikolasKKLSS2018sever} assume a type of worst-case noise for stochastic optimization where $\alpha$-fraction of the sampled funct, but requires access to the original samples and functions. Relies on down-weighting specific points and functions, we cannot do this here since we get only access to noisy gradients at every step. Also they only tolerate a small constant fraction of corruptions, we tolerate a vanishingly small fraction of corruptions.


\paragraph{Robust Estimation}
Our oblivious noise oracle for optimization is motivated by the recent work on regression under oblivious outliers.
In the case of linear regression, the oblivious noise model can be seen as the weakest possible noise model that allows almost all points to be arbitrarily corrupted, while still allowing for recovery of the true function with vanishing error~\cite{BhatiaJK15, suggala2019adaptive}. 
This also captures heavy-tailed noise that may not have any moments.
The setting has been studied for various problems, including  regression~\cite{pesme2020online, diakonikolas2023oblivious}, PCA~\cite{d2021consistent}, and sparse signal recovery~\cite{SoSOblivious21}.

On the other hand, there has been a flurry of work on robust estimation in regards to worst-case adversarial outliers (see, e.g.,~\cite{DKKLMS16, LaiRV16, CSV17, DiakonikolasKKLSS2018sever}). 
% Most notably, our paper makes use of algorithms for robust mean estimation and list-decodable mean estimation. 
Robust mean estimation aims to develop an efficient mean estimator when $(1-\alpha)$-fraction of the samples is arbitrary. In contrast, list-decodable mean estimation generates a small list of candidates such that one of these candidates is a good estimator. While robust mean estimation becomes information-theoretically impossible when $\alpha \le 1/2$, the relaxation to output a list allows the problem to become tractable for any $\alpha \in (0,1]$~\cite{CSV17, diakonikolas2022list}.
See~\cite{DK19-survey, DK23-book} for in-depth treatments of the subject.

In the past, robust mean estimators have been used to perform robust
gradient estimation (see, e.g.,~\cite{CSV17, DiakonikolasKKLSS2018sever}),
which is similar to what we do in our paper.
However, these results assume access to the entire function set, which allows them to discard outlier functions.
In contrast, in our setting, we only have access to a noisy gradient oracle, so
at each step, we get a fresh sample set and, hence, a different set of outliers. This introduces further difficulties 
, which we resolve via location estimation.

We note a subtle difference in the standard list-decodable 
mean estimation setting and the setting considered in this work.
The standard list-decodable mean estimation setting draws 
an inlier with probability $\alpha$ and an outlier with the remaining probability. 
In contrast, our model gets samples of the kind $\xi + z$ where $z$ is drawn from the inlier distribution,
and $\Pr[\xi = 0] > \alpha$, and is arbitrary otherwise.
The algorithms for the mixture setting continue to work in our setting as well. Another difference is that the standard setting requires that the distribution have bounded variance \emph{in every direction}. On the other hand, in the optimization literature, the assumption is that the stochastic gradient has bounded expected squared \emph{norm}  from the expectation. 
% \snote{also need to discuss the difference with standard robust statistics, in the sense the objective is different?}



\paragraph{Location estimation}

Location estimation has been extensively studied since the 1960s. 
Traditional approaches to location estimation have focused on 
achieving optimal estimators in the asymptotic regime. 
The asymptotic theory of location estimation is discussed in detail in~\cite{van2000asymptotic}. 

Recent research has attempted to develop the finite-sample theory of location estimation. 
These efforts aim to estimate the location of a Gaussian-smoothed distribution 
with a sample complexity that matches the optimal sample complexity \new{up to the sharp constant} 
(see \cite{gupta2022finite} and \cite{gupta2023high}).
However, these results assume prior knowledge of the 
likelihood function of the distribution up to translation (incidentally, this is the only setting where the optimal fisher-information rate is actually possible). 

Another closely related work initiates the study of robust location estimation for the case
where the underlying high-dimensional distribution is symmetric
and an $0 < \eps \ll 1/2$ fraction of the samples are adversarially corrupted \cite{novikov2023robust}.
This follows the line of work on robust mean estimation discussed above. 

We present a finite-sample guarantee for the setting with
noisy access to samples drawn from a distribution and its translation.
Our assumption on the distribution is that it places an $\alpha$ mass at some point, 
where $\alpha \in (0, 1)$ and, for instance, could be as small as $1/d^c$ for some constant $c$.
The noise is constrained to have mean zero and bounded variance,
but crucially the noise added to the samples coming from the distribution
and its translation might be drawn from \emph{different distributions}. 
To the best of our knowledge, this is the first result
that has noisy access, does not have prior knowledge of
the probability density of the distribution and achieves a finite-sample guarantee.
% Also, $\alpha$ can be as small as $1/d^C$, with $C$ being a constant. 
% \snote{Is this better? we likely need a lot more content.. but unclear if there is any other
% finite sample work out there that doesn't try to get optimal results..}


